Automated Evaluation of Personalized Text Generation using Large Language Models

Personalized text generation presents a specialized mechanism for delivering content that is specific to a user's personal context. While the research progress in this area has been rapid, evaluation still presents a challenge. Traditional automated metrics such as BLEU and ROUGE primarily measure lexical similarity to human-written references, and are not able to distinguish personalization from other subtle semantic aspects, thus falling short of capturing the nuances of personalized generated content quality. On the other hand, human judgments are costly to obtain, especially in the realm of personalized evaluation. Inspired by these challenges, we explore the use of large language models (LLMs) for evaluating personalized text generation, and examine their ability to understand nuanced user context. We present AuPEL, a novel evaluation method that distills three major semantic aspects of the generated text: personalization, quality and relevance, and automatically measures these aspects. To validate the effectiveness of AuPEL, we design carefully controlled experiments and compare the accuracy of the evaluation judgments made by LLMs versus that of judgements made by human annotators, and conduct rigorous analyses of the consistency and sensitivity of the proposed metric. We find that, compared to existing evaluation metrics, AuPEL not only distinguishes and ranks models based on their personalization abilities more accurately, but also presents commendable consistency and efficiency for this task. Our work suggests that using LLMs as the evaluators of personalized text generation is superior to traditional text similarity metrics, even though interesting new challenges still remain.

==> subfiles/exp_copy.tex <==
% \noindent control study 
% \noindent Consistency of evaluation
% \noindent Case study (w/ explanation)
% \noindent Different models as Evaluator (24b and 340b on the human eval dataset)


\section{Experimental Setup}

\subsection{Datasets}
%\noindent\textbf{Datasets.} 

We study personalized text generation evaluation  on six public datasets, where four of them are based on Amazon reviews, one is from Reddit, and the other is from the email domain. The Amazon review data~\cite{ni2019justifying} encompasses user reviews spanning various product categories. Specifically, we designate the user reviews in categories of \textit{home}, \textit{movie}, \textit{clothing}, and \textit{books} as four separate datasets.  The Reddit comments dataset~\cite{reddit2015} consists of all the posts and comments available on Reddit from 2007 to 2015. The Avocado Research Email Collection~\cite{oard2015avocado} includes emails and attachments sourced from $279$ accounts of an IT company, "Avocado".  We follow the processing steps of LaMP~\cite{salemi2023lamp} to organize emails by sender addresses, which exceeds $279$ accounts as there may be external senders. For all the six datasets, we deduplicate identical documents from each user's personal context. To construct immediate context $Q_t$, user profile $U_t$ and $\tilde{X}_t$, we follow the processing step of \cite{li2023teach}. We treat review title and product description as immediate context $Q_t$ on amazon review dataset, and treat reddit post and avocado email title as immediate context $Q_t$ on Reddit and Avocado email datasets respectively.  For all the datasets, we leverage past examples write by the same user $t$ as user profile $U_t$. Given user $t$, amazon review content, reddit post content and avocado email context (excluding the title) are used as $\tilde{X}_t$. More information about datasets can be found in the appendix section. 

% \textcolor{red}{QM: Need data statistics. We also need to describe how we construct $Q$, $U_t$, and $\tilde{X}_t$ here. Maybe cite Cheng et al., 2023 if the same strategy is used?} 
\vspace{-0.1in}
\subsection{Generators and Evaluators} 

There are two types of models in our experiment: one for generating the personalized text (generators) and one for evaluating the generation models (evaluators). 

For the \textbf{Generators}, we experiment with the T5 family of checkpoints, including T5-XXL (XXL), T5-XL (XL), T5-Large, and T5-Base. We choose these T5 models because they offer a range of open-sourced checkpoints from hundreds of millions to tens of billions of parameters, enabling in-depth study across various model sizes and capabilities. %By evaluating performance variances through human judgments and targeted experiments, we can thoroughly analyze how model scale impacts personalized text generation. 
%The diverse T5 model family provides a decent testbed to uncover insights across model capabilities. 
We finetune T5 checkpoints using a training split of each dataset, using personal contexts $U_t$ and immediate context $Q$ as input and the user written text $\tilde{X}_t$ as target.  We also include PALM-IT-S in the PaLM-2 model family~\cite{anil2023palm} for one specific experiment when contrasting human and LLM evaluations.  %to show potential mixed performance in multi-faceted assessments.  
Note that the user written text $\tilde{X}_t$ can also be seen as generated from a hypothetical gold-standard model (denoted as ``GOLD'' thereafter), which we also include for comparison.  

For the \textbf{Evaluators}, we use PALM-IT-L in the PaLM-2 model family~\cite{anil2023palm} as default unless indicated otherwise. For each pair of generated examples ($\hat{X}^a_t$ and $\hat{X}^b_t$), we repeat the evaluation 40 times, with $\hat{X}^a_t$ following $\hat{X}^b_t$ in half of the runs and vice versa to mitigate the order bias. For comparison purposes, we also include a series of evaluators that are not based on LLMs: Human, %(described in Section~\ref{sec:human-evaluator}),
BLEU, ROUGE-1, ROUGE-2, and ROUGE-L. The latter four evaluators use conventional NLG metrics to decide which output example, $\hat{X}^a_t$ or $\hat{X}^b_t$, has a better match to the hypothetical gold standard $\tilde{X}_t$. 



\input{subfiles/human_eval}


\section{Evaluate the Evaluators}

\input{subfiles/compare_human_autorater}

\input{subfiles/consistency}


\begin{table*}[!h]
  \centering
    \caption{Overall evaluation results of multiple T5 generators with {\sysname} Elo Ratings and average scores of traditional NLG Metrics over all datasets. P, Q, and R stand for Personalization, Quality and Relevance respectively. The Elo ratings are median numbers from 1000 bootstrap rounds to minimize the sample order effect in Elo rating system.}
    	\vspace{-0.1in}
  \resizebox{0.7\linewidth}{!}{%
  \begin{tabular}{l|c|c|c|c|c|c|c|c}
    \hline
    \multirow{2}{*}{\textbf{Generator Model}} & \multicolumn{4}{c|}{\textbf{{\sysname} Elo Metrics}} &  \multicolumn{4}{c}{\textbf{Traditional NLG Metrics}} \\
    \cline{2-9}
    & \textbf{P Elo} & \textbf{Q Elo} & \textbf{R Elo} & \textbf{Overall Elo} & \textbf{BLEU} & \textbf{ROUGE-1} & \textbf{ROUGE-2} & \textbf{ROUGE-L}   \\
    \hline
    T5 XXL & 1140 & 1174 & 1110 & 1140& 5.98&29.59&8.21&18.76  \\
    \hline
    T5 XL & 1031 & 1036 &  1018 & 1027& 5.78	& 27.05& 	7.60&	17.89 \\
    \hline
    T5 Large & 953 & 942 & 968 &955& 4.89 &	24.97 &	6.39&	16.77  \\
    \hline
    T5 Base & 876 & 849 &  904 & 878 & 5.19	& 23.63	& 6.57&	16.83 \\
    \hline
  \end{tabular}
  }
  \label{tab:t5_elo_bleu_evaluation}
  \vspace{-0.1in}
\end{table*}



\subsection{Generator-level Evaluations}
%\noindent\textbf{Size of evaluation samples.} 

The previous sections validate the accuracy, consistency, and sensitivity of the evaluators at a micro-level, investigating their decisions on each sampled test case. We continue to validate the performance of the evaluators at a macro-level, by looking at how they prefer different generators as a whole rather than individual test cases. When comparing two generators, %pairwise across four Amazon review, Reddit and Avocado datasets, 
we randomly sample 1,000 test cases from each dataset for comparison unless otherwise specified. %, the settings remain consistent.

\noindent\textbf{AuPEL Elo Ranking vs. Generator Size.} Table \ref{tab:t5_elo_bleu_evaluation} presents the Elo ratings of various T5 models using {\sysname} metrics, compared with the average ratings using traditional NLG metrics. Elo ratings are calculated for personalization, quality, and relevance separately, and an Overall Elo rating is computed aggregating all three dimensions (considering three ``games'' played per test case). Intuitively, under all four Elo ratings, a larger T5 model is always rated higher than a smaller T5 model. The Elo ratings are also smoothly distributed, with a relatively consistent gap between two consecutive T5 checkpoints. Ratings based on the traditional NLG metrics are less intuitive. In particular, T5-Large has been ranked the lowest by BLEU, ROUGE-2, and ROUGE-L, lower than T5-Base that has only one third parameters. 


%and median numbers of Elo ratings are reported from a bootstrap of 1000 rounds.  
%One salient observation from this table is the hierarchical performance in the Elo ratings, indicating a clear differentiation among the models. Specifically, the T5 XXL model outperforms the others in all three Elo categories, confirming its superior capability. Such Elo ratings based on the LLM evaluation provide a reliable ranking of a model's capability in terms of flexibly defined dimensions of interest. Notably, the Elo system grants researchers the advantage of evaluating LLM capabilities on various dimensions without the necessity of ground truth. This makes it particularly robust, especially when compared to traditional NLP metrics such as BLEU and Rouge. In the context of BLEU and Rouge scores, it's evident that these metrics, which mainly estimate similarity between generated text and a given ground truth, may not always align with intuitive perceptions of model capability. This is particularly evident when comparing the T5 Large and T5 Base models. Despite T5 Large being presumably more capable, its scores, especially in terms of BLEU and Rouge1, are mixed, underscoring the limitations of these metrics, especially in creative, personalized generation scenarios where ground truth is not singularly defined.

%\input{subfiles/results_blue_rouge}


% \begin{figure}[!hbt] 
% \centering   
% \includegraphics[width=.47\textwidth]{figs/books_consistency.png} 
% \label{fig:consistency}
% \caption{.}  
% \end{figure}



% \begin{table}[!h]
% \centering
% \caption{Pairwise evaluation results across various T5 checkpoints on Amazon book dataset.}
% \resizebox{0.8\linewidth}{!}{
% \begin{tabular}{c|c|c|c|c|c}
% \hline
% Model a & Model b & Eval Dim & Win & Loss & Tie \\
% \hline
% \multirow{9}{*}{xxl} & xl & Personalization & 62.6 & 32.4 & 5.0 \\
% & xl & Quality & 66.5 & 31.4 & 2.1 \\
% & xl & Relevance & 61.8 & 32.2 & 6.0 \\
% \cline{2-6}
% & large & Personalization & 74.9 & 21.8 & 3.3 \\
% & large & Quality & 80.4 & 19.2 & 0.4 \\
% & large & Relevance & 70.4 & 24.5 & 5.1 \\
% \cline{2-6}
% & base & Personalization & 77.8 & 19.4 & 2.8 \\
% & base & Quality & 83.7 & 15.7 & 0.6 \\
% & base & Relevance & 75.3 & 20.6 & 4.1 \\
% \midrule
% \multirow{6}{*}{xl} & large & Personalization & 62.6 & 32.6 & 4.8 \\
% & large & Quality & 68.2 & 29.7 & 2.1 \\
% & large & Relevance & 59.5 & 34.1 & 6.4 \\
% \cline{2-6}
% & base & Personalization & 68.3 & 27.5 & 4.2 \\
% & base & Quality & 73.4 & 25.6 & 1.0 \\
% & base & Relevance & 63.5 & 31.7 & 4.8 \\
% \midrule
% \multirow{3}{*}{large} & base & personalization & 55.7 & 38.3 & 6.0 \\
% & base & Quality & 56.8 & 40.9 & 2.3 \\
% & base & Relevance & 52.9 & 41.0 & 6.1 \\
% \hline
% \end{tabular}}
% \label{tab:amazon_book_win_rate}
% \end{table}

\begin{table}[!h]
\centering
\caption{Head-to-head comparison records between various T5 generators on Amazon book dataset.}	\vspace{-0.1in}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c}
\hline
Model a & Model b & Eval Dim. & Win & Loss & Tie \\
\hline
\multirow{9}{*}{T5 XXL} & \multirow{3}{*}{T5 XL} & Personalization & 62.6 & 32.4 & 5.0 \\
&  & Quality & 66.5 & 31.4 & 2.1 \\
&  & Relevance & 61.8 & 32.2 & 6.0 \\
\cline{2-6}
& \multirow{3}{*}{T5 Large} & Personalization & 74.9 & 21.8 & 3.3 \\
&  & Quality & 80.4 & 19.2 & 0.4 \\
&  & Relevance & 70.4 & 24.5 & 5.1 \\
\cline{2-6}
& \multirow{3}{*}{T5 Base} & Personalization & 77.8 & 19.4 & 2.8 \\
&  & Quality & 83.7 & 15.7 & 0.6 \\
&  & Relevance & 75.3 & 20.6 & 4.1 \\
\midrule
\multirow{6}{*}{T5 XL} & \multirow{3}{*}{T5 Large} & Personalization & 62.6 & 32.6 & 4.8 \\
&  & Quality & 68.2 & 29.7 & 2.1 \\
&  & Relevance & 59.5 & 34.1 & 6.4 \\
\cline{2-6}
& \multirow{3}{*}{T5 Base} & Personalization & 68.3 & 27.5 & 4.2 \\
&  & Quality & 73.4 & 25.6 & 1.0 \\
&  & Relevance & 63.5 & 31.7 & 4.8 \\
\midrule
\multirow{3}{*}{T5 Large} & \multirow{3}{*}{T5 Base} & Personalization & 55.7 & 38.3 & 6.0 \\
&  & Quality & 56.8 & 40.9 & 2.3 \\
&  & Relevance & 52.9 & 41.0 & 6.1 \\
\hline
\end{tabular}}
\label{tab:amazon_book_win_rate}
\end{table}

% \begin{table}[!h]
% \centering
% \caption{Pairwise evaluation results across various T5 checkpoints on Reddit dataset.}
% \resizebox{0.8\linewidth}{!}{
% \begin{tabular}{c|c|c|c|c|c}
% \hline
% Model a & Model b & Eval Dim & Win & Loss & Tie \\
% \hline
% \multirow{9}{*}{xxl} & xl & personalization & 67.1 & 28.6 & 4.3 \\
% & XL & quality & 71.7 & 26.9 & 1.4 \\
% & XL & relevance & 65.4 & 29.2 & 5.4 \\
% \cline{2-6}
% & large & Personalization & 80.4 & 17.9 & 1.7 \\
% & large & Quality & 80.4 & 18.2 & 1.4 \\
% & large & Relevance & 71.0 & 24.2 & 4.8 \\
% \cline{2-6}
% & base & Personalization & 84.6 & 13.7 & 1.7 \\
% & base & Quality & 83.3 & 15.7 & 1.0 \\
% & base & Relevance & 74.4 & 21.6 & 4.0 \\
% \midrule
% \multirow{6}{*}{xl} & large & Personalization & 60.2 & 36.1 & 3.7 \\
% & large & Quality & 59.7 & 37.7 & 2.6 \\
% & large & Relevance & 51.2 & 41.1 & 7.7 \\
% \cline{2-6}
% & base & Personalization & 72.2 & 24.9 & 2.9 \\
% & base & Quality & 66.6 & 31.1 & 2.3 \\
% & base & Relevance & 59.9 & 33.8 & 6.3 \\

% \midrule
% \multirow{3}{*}{large} & base & Personalization & 59.7 & 36.7 & 3.6 \\
% & base & Quality & 59.3 & 39.3 & 1.4 \\
% & base & Relevance & 53.2 & 38.6 & 8.2 \\
% \hline
% \end{tabular}}
% \label{tab:reddit_win_rate}
% \end{table}

% \begin{table}[!h]
% \centering
% \caption{Pairwise evaluation results across various T5 checkpoints on Reddit dataset.}
% \resizebox{0.8\linewidth}{!}{
% \begin{tabular}{c|c|c|c|c|c}
% \hline
% Model a & Model b & Eval Dim & Win & Loss & Tie \\
% \hline
% \multirow{9}{*}{T5 XXL} & \multirow{3}{*}{T5 XL} & Personalization & 67.1 & 28.6 & 4.3 \\
% &  & Quality & 71.7 & 26.9 & 1.4 \\
% &  & Relevance & 65.4 & 29.2 & 5.4 \\
% \cline{2-6}
% & \multirow{3}{*}{T5 Large} & Personalization & 80.4 & 17.9 & 1.7 \\
% & & Quality & 80.4 & 18.2 & 1.4 \\
% & & Relevance & 71.0 & 24.2 & 4.8 \\
% \cline{2-6}
% & \multirow{3}{*}{T5 Base} & Personalization & 84.6 & 13.7 & 1.7 \\
% &  & Quality & 83.3 & 15.7 & 1.0 \\
% & & Relevance & 74.4 & 21.6 & 4.0 \\
% \midrule
% \multirow{6}{*}{T5 XL} & \multirow{3}{*}{T5 Large} & Personalization & 60.2 & 36.1 & 3.7 \\
% &  & Quality & 59.7 & 37.7 & 2.6 \\
% & & Relevance & 51.2 & 41.1 & 7.7 \\
% \cline{2-6}
% & \multirow{3}{*}{T5 Base} & Personalization & 72.2 & 24.9 & 2.9 \\
% & & Quality & 66.6 & 31.1 & 2.3 \\
% & & Relevance & 59.9 & 33.8 & 6.3 \\
% \midrule
% \multirow{3}{*}{T5 Large} & \multirow{3}{*}{T5 Base} & Personalization & 59.7 & 36.7 & 3.6 \\
% & & Quality & 59.3 & 39.3 & 1.4 \\
% & & Relevance & 53.2 & 38.6 & 8.2 \\
% \hline
% \end{tabular}}
% \label{tab:reddit_win_rate}
% \end{table}


\noindent\textbf{Head-to-head records between T5 checkpoints.} Tables \ref{tab:amazon_book_win_rate} %displays the reliability and sensitivity of leveraging LLM evaluation on Amazon Books. More results are included in Appendix Section. From the table, a clear and consistent hierarchy in model capability emerges. T5 XXL is ranked as the most capable model, followed by T5 XL, T5 Large, and lastly, T5 Base. The tables 
presents the head-to-head contest records between different T5 models in all three evaluation dimensions on one of the datasets (more results are included in Appendix). We see that when a generator model competes with another model smaller in size (and with a lower Elo rating), it has a higher winning rate. When the gap of Elo rating is larger, the winning rate increases. The LLM evaluator adeptly captures the degree of improvement a larger generator model brings compared to its smaller counterpart across all three evaluation dimensions. %For instance, the win rate of T5 XXL over T5 XL in terms of personalization on Amazon Books is 62.6\%. This win rate increases to 74.9\% when compared with T5 Large and further to 77.8\% with T5 Base. This trend is consistently observed, affirming the reliability of {\sysname}.

\subsection{Ablation Study}
Either at the test case level or at the generator level, {\sysname}'s evaluations on the three dimensions, quality, relevance, and personalization are more or less correlated. This is intuitive, as a more capable generator is likely to be better at all these aspects: writing fluently, keeping to the point, and mimicking an author. However, are these dimensions indeed measuring the relevance and personalization of the generated text, or are they just a variant of the general quality? To validate that the three dimensions of {\sysname} are measuring what they are supposed to measure, we conduct controlled experiments and test whether {\sysname} scores are indeed influenced by the nuanced differences between quality, relevance, and personalization (as defined in \ref{sec:multifacet}).  


\begin{table}[!h]
\vspace{-0.1in}
	\caption{Ablation study by swapping user's personal context in generation. Original generator vs. ablated generator. Swapping personal context hurts personalization. }	\vspace{-0.1in}
	\begin{center}
\resizebox{0.7\linewidth}{!}{\begin{tabular}{l|c|lc c cc}
		\toprule \bf Dataset & Eval Dim. & Win & Loss & Tie \\ 
		\midrule
		\multirow{3}{*}{\bf Amazon books} 
		& Personalization & 64.2 & 30.8 & 5.0 \\
		& Quality & 54.6 & 44.2 & 1.2 \\
		& Relevance & 54.8 & 43.1 & 2.1 \\ 
		\midrule
		\multirow{3}{*}{\bf Amazon clothing} 
		& Personalization & 70.3 & 22.3 & 7.4 \\
		& Quality & 49.2 & 49.0 & 1.8 \\
		& Relevance & 72.0 & 26.5 & 1.5 \\ 
		\midrule
		\multirow{3}{*}{\bf Amazon home} 
		& Personalization & 65.5 & 28.9 & 5.6 \\
		& Quality & 50.8 & 47.4 & 1.8 \\
		& Relevance & 50.5 & 46.7 & 2.8 \\ 
		\midrule
		\multirow{3}{*}{\bf Amazon movie} 
		& Personalization & 69.0 & 27.7 & 3.3 \\
		& Quality & 54.6 & 43.6 & 1.8 \\
		& Relevance & 54.0 & 44.8 & 1.2 \\ 
		\midrule
		\multirow{3}{*}{\bf Reddit} 
		& Personalization & 57.2 & 36.3 & 6.5 \\
		& Quality & 51.1 & 46.1 & 2.8 \\
		& Relevance & 54.0 & 42.3 & 3.7 \\ 
		\midrule
		\multirow{3}{*}{\bf Avocado email} 
		& Personalization & 83.4 & 14.7 & 1.9\\
		& Quality & 61.1 & 37.4 & 1.4 \\
		& Relevance & 51.7 & 44.5 & 3.8  \\ 
		\midrule
\end{tabular}}
	\end{center}
\label{tab:ablation_user_history}
\vspace{-0.1in}
\end{table}

\noindent\textbf{Ablation study on personal context.} As personalization is evaluated by {\sysname}$_P$($\hat{X}^a_t$, $\hat{X}^b_t$ | $U_t$), a text example generated under a different user context $U_{t'}$ should not be as personalized (for the target user $t$) as the example generated under the target user's own context $U_t$, when all other conditions are identical. To verify this, we construct an ablated generator that uses the same T5 XXL model and test cases except for randomly swapping the user's historical writing examples with those of another user's. Table~\ref{tab:ablation_user_history} presents ablation results of how manipulating the user's writing history impacts generation quality. We see that the original generator has a close to 50-50 win rate against the ablated generator on quality and relevance, which is reasonable as everything except for $U_t$ is controlled. The ablated generator does slightly worse in some cases, possibly because the LLM generator gets confused by the mismatch between the immediate context $Q$ (which is also composed by the user $t$) and the swapped user context $U_{t'}$.  As expected, the original model obtains a clearly higher win rate in personalization over the ablated generator,  ranging from 57-83\%. This indicates that the personal context provided to the LLM generator has a significant influence on how much the output is personalized, and this influence is captured by {\sysname}'s personalization evaluation. %This aligns with the fact that the user's prior writing provides more information about their unique style. %For relevance and quality, the win rates are closer to 50-50 when modifying user profile broadly.  These results align with our expectations that user profile significantly influences personalization but has minimal effect on quality and relevance. The reliably higher personalization win rates demonstrate that the LLM evaluators can effectively identify improved capturing of user style when better immediate context is provided. 

\begin{table}[!h]
	\caption{Ablation study by swapping immediate context (Title and start of text) in generation. Original generator vs. ablated generator. Swapping immediate context destroys relevance and moderately reduces personalization.}  %assessing the effects of varying immediate context for text generation. Note that immediate context, such as review titles or Reddit post titles, inherently embody user writing style and opinion, which are also captured by the evaluation.}
	\vspace{-0.1in}
	\begin{center}
	\resizebox{0.7\linewidth}{!}{
		\begin{tabular}{l|c|lc c cc}
			\toprule \bf Dataset & Eval Dim. &Win & Loss & Tie       \\ \midrule

		    \multirow{3}{*}{\bf Amazon books} &  Personalization & 68.3 & 28.7 & 3.0 \\
		& Quality & 54.7 & 44.5 & 0.8 \\
		& Relevance & 96.1 & 3.6 & 0.3 \\ 
		    \midrule
		      \multirow{3}{*}{\bf Amazon clothing} 	& Personalization & 61.1 & 34.0 & 4.9 \\
		& Quality & 47.1 & 50.3 & 2.6 \\
		& Relevance & 99.4 & 0.6 & 0.0 \\ 
		    \midrule
		       \multirow{3}{*}{\bf Amazon home} &  Personalization & 59.4 & 34.8 & 5.8 \\
		& Quality & 49.4 & 48.5 & 2.1 \\
		& Relevance & 99.9 & 0.1 & 0.0 \\ 
		    \midrule
		        \multirow{3}{*}{\bf Amazon movie} &   Personalization & 57.3 & 39.2 & 3.5 \\
		& Quality & 52.4 & 46.1 & 1.5 \\
		& Relevance & 87.7 & 11.2 & 1.1 \\ 
		 \midrule
		       \multirow{3}{*}{\bf Reddit} & Personalization & 92.8 & 6.2 & 1.0 \\
		& Quality & 51.5 & 47.2 & 1.3 \\
		& Relevance & 97.0 & 2.7 & 0.3 \\ 
		    \midrule
		       \multirow{3}{*}{\bf Avocado email} & Personalization & 70.6 & 23.7 & 5.7\\
		    & Quality& 55.9 & 42.2 & 1.9\\
		    & Relevance & 98.6 & 1.4 & 0.0 \\ 

			\bottomrule
		\end{tabular}}
	\end{center}
\label{tab:ablation_context}
\vspace{-0.15in}
\end{table}

\noindent \textbf{Ablation study on immediate context.} Similarly, as personalization is evaluated by {\sysname}$_P$($\hat{X}^a_t$, $\hat{X}^b_t$ | $Q$), a text example generated given a different immediate context $Q'$ should not be as relevant to the original query $Q$, when all other conditions are identical. To verify this, we ablate the T5 XXL generator by randomly swapping the immediate context $Q$ in a test case with one from another test case, while all other conditions are controlled. Table~\ref{tab:ablation_context} presents the win-loss ratio of the original generator against the ablated generator. %from an ablation study evaluating the impact of providing relevant immediate context on various generation quality metrics. Based on the study design, 
We see that while the win rates on quality are close to 50-50, the original generator has a dominating winning record on relevance, as we expected.  %expect to see higher win rates for relevance and personalization when comparing generations with and without relevant immediate context. This is because the immediate context, such as article titles, provides topical information and captures distinctive aspects of the user's writing style. For quality, we anticipate more mixed results since the same T5 XXL model is used for generation. The results align well with these expectations. For relevance, win rates range from 87-100\% across datasets when immediate context is provided, indicating the model generates more topically relevant responses. 
Interestingly, we also see inflated win rates on personalization, although not as significant as those on relevance. This is because the immediate contexts in our case are the titles or starting sentences of the reviews or emails, which also encodes some information about the author's writing styles. Swapping it with that of another author could also make the generated text less personalized. Nevertheless, the personal context $U_t$ contains more useful information than the immediate context, and the ablated generator is still able to generate texts in the user's voice but completely irrelevant.  This result verifies that {\sysname}'s relevance and personalization evaluations do capture the nuances in these two aspects that are separated from the general text quality. %showing that the immediate context is helpful to provide user writing style and opinion information.  In contrast, quality results are more evenly split between wins and losses when changing context given the same underlying model. Overall, this demonstrates the LLMs reliably distinguish differences in these key evaluation dimensions.  This reliability helps validate LLMs for automated evaluation, reducing the need for expensive human evaluation.




\subsection{Emerging ability of LLM Evaluators }




% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.4\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/book_sensitivity_R.png} 
%         \caption{Amazon Books}
%         \label{fig:sub1}
%     \end{subfigure}
%     \hfill % or \quad or \hspace{5mm} or some space
%     \begin{subfigure}[b]{0.4\textwidth}
%         \centering
%       \includegraphics[width=\textwidth]{figs/reddit_sensitivity_R.png} 
%         \caption{Reddit}
%         \label{fig:sub2}
%     \end{subfigure}
%     \caption{Sensitivity Analysis}
%     \label{fig:main}
% \end{figure}








\begin{figure}[!h]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/p_win_loss_tie.png} 
        \caption{Personalization}
        \label{fig:sub1}
    \end{subfigure}
    \hfill % or \quad or \hspace{5mm} or some space
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
       \includegraphics[width=\textwidth]{figs/q_win_loss_tie.png}
        \caption{Quality}
        \label{fig:sub2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
       \includegraphics[width=\textwidth]{figs/r_win_loss_tie.png} 
        \caption{Relevance}
        \label{fig:sub2}
    \end{subfigure}
    \caption{Pairwise comparison of multiple T5 generators using PaLM-IT-L and PaLM-IT-S as evaluators. The Tie-rate in Personalization is significantly higher when switching from PaLM-IT-L to PaLM-IT-S while the evaluations of Quality and Relevance are not significantly affected by the switch. }
    \label{fig:it_l_s}
    
\end{figure}

%\noindent\textbf{Emerging ability in personalized text generation evaluation.}  
We also examine the use of different LLMs as the evaluator, in particular PaLM 2-L-IT versus PaLM-2-S-IT, to compare the T5-XXL generator with three other generator models: T5-XL, T5-Large, and T5-Base. Figure~\ref{fig:it_l_s} shows the Win-Loss-Tie rates in personalziation, quality, and relevance for every matched pair. PaLM 2-L-IT and PaLM-2-S-IT produce similar evaluation results in terms of quality and relevance, showing the highest win rate when T5-XXL competes against Base, followed by a lower win rate against T5-Large and an even lower win rate against T5-XL (but still higher than 60\%). The two evaluators however produce very different result on personalization. PaLM-2-L-IT's judgments on personalization are similar to those on the other two dimensions, while PaLM-2-S-IT outputs much lower win rates in all three match-ups, as well as over 30\% of ties. %higher win rate when comparing different model pairs but around 30\% of comparisions are judged as tie while percentage of ties is much lower when using PaLM-2-L-IT. 
This indicates that while the smaller evaluator PaLM-2-S-IT is as capable as the larger model to evaluate quality and relevance, it struggles to accurately assess personalziation, which is more subtle and subjective. As the size of the evaluator model grows, the ability of evaluating personalization emerges. 


\begin{table}[!h]
\centering
\caption{Pairwise comparison of PaLM 2-S-IT and Gold Standard (Human generator) on Amazon book dataset.}	\vspace{-0.1in}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c}
\hline
Model a & Model b & Eval Dim & Win & Loss & Tie \\
\hline
\multirow{3}{*}{PaLM 2-S-IT} &  & personalization & 8.6 & 89.2 & 2.2 \\
& Human & quality & 75.5 & 23.0 & 1.5 \\
&  & relevance &28.3 & 68.7 & 3.0 \\
\hline
\end{tabular}}
\label{tab:amazon_book_win_rate_w_human}
\vspace{-0.1in}
\end{table}

\subsection{Limits of LLM Generator}

With the multi-faceted evaluation, we are also able to delve into the fine-grained aspects of the ability of LLM generators, so that we can better understand their limits. We use PaLM 2-S-IT as our generation model and prompt it in a zero-shot manner. The results in Table~\ref{tab:amazon_book_win_rate_w_human} indicate that PaLM 2-S-IT obtains a high win rate (75.5\%) in \textit{quality} against the human written examples (GOLD generator). %As expected, PaLM 2-S-IT lagged far behind humans in terms of personalization and relevance due to a zero-shot nature of generation. 
However, we can see that the \textit{relevance} and especially the degree of \textit{personalization} of the text generated by the LLM still trails human-written text by a large margin. Traditional NLG metrics fail to capture these nuanced differences, but multi-faceted evaluation provides fine-grained insights on the limits of the writing ability of the LLMs. %into the remaining gaps between large language models like PaLM 2-S-IT, and human writing ability.



==> subfiles/method_backup.tex <==
\vspace{-0.1in}
\section{Methodology}
In this section, we propose a novel evaluation method, {\sysname}. We begin with a formal definition of the personalized text generation task and its automated evaluation. We then delve into the multiple dimensions that are essential for assessing the goodness of the generated output. Among these dimensions, \textit{personalization} is particularly subjective and challenging to measure. To provide a foundation for automated evaluation, we relate the subjective personalized evaluation with the objective author attribution problem. Finally, we present how to utilize LLM for a multi-faceted evaluation of personalized text generation.

\subsection{Automated Evaluation of Personalized Text Generation}

\noindent\textbf{Personalized text generation.} Following prior literature \cite{li2023teach}, we define the problem of personalized text generation as: \textit{generating a piece of text relevant to a given context in a personalized voice,  taking into account the user's personal context}. Formally, given the target user $t$, let $U_t$ be the user's \textit{personal context} (a.k.a. user profile, history, or preferences in specific application scenarios), often observed. Denote the \textit{immediate context} of the generation task, e.g., a topic of interest, a query, or a prompt, as $Q$. Let $X_t$ be the text the target user $t$ is anticipated to generate under contexts $Q$ and $U_t$ (the groundtruth). The personalized text generation process can be described as $\hat{X}_t = G(U_t, Q)$, where $G(\cdot)$ stands for a generation model and $\hat{X}_t$ is the actual text generated by the model. In reality, the groundtruth $X_t$ is often not observable, and one needs to evaluate the goodness of $\hat{X}_t$ without comparing it to the groundtruth.  

\noindent\textbf{Automated evaluation.} %Automated evaluation is a critical research question for personalized text generation. 
When the groundtruth $X_t$ is not available for an ad hoc query $Q$ or a specific user $t$, one can still evaluate the generated output $\hat{X}_t$ through human annotations or an A/B test. These ``manual'' evaluations require considerable human effort and are costly to conduct in reality. We define an \textit{automated} evaluation as a procedure where no user study or field experiment (A/B Test) is involved, and the evaluation metrics are calculated algorithmically. Widely used automated metrics for text generation include text overlap metrics such as BLEU and ROUGE, text quality metrics such as coherence, or task-based metrics such as classification accuracy. All of those are often done by comparing the model-generated text $\hat{X}$ with a reference text $\tilde{X}$, often pre-curated by humans and treated as a surrogate of the groundtruth $X$. In personalized text generation, acquiring a surrogate groundtruth for specific users, represented as $\tilde{X}_t$, poses a challenge. Moreover, even if $\tilde{X}_t$ is secured, merely computing the similarity between $\tilde{X}_t$ and $\hat{X}_t$ fails to capture the subtle distinctions in the degree of personalization, especially when confounded with other aspects such as the generic quality of $\hat{X}_t$ or the relevance between $\hat{X}_t$ and $Q$.  {\sysname} explores a different path by leveraging a large language model to automatically assess pre-defined dimensions of the goodness of $\hat{X}_t$, without the need for  groundtruth $X_t$ or the reference $\tilde{X}_t$.  %interests to unveil the performance evaluation flexibility in naunced aspects and relax the strong dependency on human generated text. The proposed evaluation system is denoted as {\sysname}.

\subsection{Multi-faceted Evaluation}
\label{sec:multifacet}
%To construct a comprehensive evaluation approach that takes into account multiple dimensions or facets of a system's performance, the proposed  evaluation method assesses a system's performance across several relevant parameters or criteria, offering a more holistic view of its capabilities and areas of improvement. 
For personalized text generation, there are multiple aspects that are related to the goodness of the output $\hat{X}_t$, including the \textit{quality} of the text $\hat{X}_t$, the \textit{relevance} between $\hat{X}_t$ and the immediate context $Q$, and the degree of \textit{personalization} regarding to the personal context $U_t$. These aspects often interleaves with each other and are hard to separate using existing NLP metrics. Below we formally define these nuanced dimensions and separate them from each other. %as three vital evaluation dimensions for personalized text generation task.

\noindent \textbf{Quality.} The overall quality measures how good the generated text (i.e., $\hat{X}_t$) is in general, independent of other contexts ($Q$ or $U_t$). This dimension captures whether the generated output is coherent, fluent, grammatically correct, or whether it looks like a piece of text written by a human \cite{garbacea2019judge}.  In personalized text generation, the overall quality of the generated output should not be compromised when $Q$ and $U_t$ are considered.  

\noindent \textbf{Relevance.} The relevance measures how relevant the generated text ($\hat{X}_t$) is to the given immediate context $Q$. Whether or not a generated text is personalized, it should remain relevant to the topic of concern, the instructions, or the immediate needs of the user. %Personalized content needs to be relevant to the user's current context, needs, or queries.
For example, when assisting a user to write a book review, talking about how this user's 2-year old daughter likes a toy is certainly ``personalized'' but is not relevant to the user's immediate need. 
%Irrelevant content, for instance,  given the immediate context of writing a review about a book, generating a review about how this user's 2-year old son is happy about a toy for toddlers is certainly personalized, would not serve the user effectively. 
 
\noindent \textbf{Personalization.}  The degree of personalization measures to what extent the generated text $\hat{X}_t$ aligns with, or is tailored to, the specific attributes, preferences, writing style, and other behaviors encapsulated within a user's profile or personal context $U_t$. Personalization serves as a distinguishing factor between a generic piece of relevant content and one that is not only relevant but also tailored for a specific individual or group. As the name suggests, this dimension is the central concern of personalized text generation.  %In the context of evaluating a personalized text generation system, it is crucial to ascertain if the system can genuinely produce content that feels individualized. 

As a high quality ensures the generated text is coherent and human readable, a high relevance ensures it satisfies the immediate information need, and a high level of personalization ensures the content is tailored to the user's personal preferences. %, and relevance ensures it aligns with the user's context and needs. 
Together, these three dimensions provide a comprehensive lens that captures the nuances of the effectiveness of personalized text generation systems, and they form the fundamentals of {\sysname}. 

\subsection{Author Attribution as a Proxy for Personalization Evaluation}

Compared to quality and relevance, the evaluation of personalization is inherently more challenging due to the subjective nature of individual preferences. 
%Evaluating personalization in text generation is inherently challenging due to the subjective nature of individual preferences. Personalization is inherently subjective. 
What might be highly personalized to one individual could seem generic or deviated to a different person, making it hard to be evaluated by human judges that are not the target user. %This variance complicates the establishment of a universal ground truth, making it difficult for traditional metrics to measure the effectiveness of personalized content. 
Moreover, personalization itself encompasses multiple nuanced aspects, from the vocabulary use to the tone and from the writing style to the ideology. Different users may prioritize these aspects differently, adding another layer of complexity to the evaluation process. Instead of enumerating these subjective aspects, we transform personalization evaluation into an author attribution problem, as it provides an objective measure of how likely a content was generated by a particular user. Author attribution is formulated as a function $\text{AA}(X, t)$ that outputs a binary prediction of whether or not the input text $X$ was written by the author $t$. With a sufficiently accurate author attribution function, $\hat{X}_t$ is considered highly personalized if there is a high probability that $\text{AA}(\hat{X}_t, t) = 1$. 

% \noindent \textbf{Fundamental Overlap.} At its core, both personalization and author attribution aim to identify unique characteristics in text. Personalization focuses on tailoring content to a specific user's preferences, history, or profile, while author attribution seeks to determine the likely authorship of a piece of text based on stylistic and content-based cues. Hence, evaluating how well a model can imitate or capture a user's style is conceptually akin to determining if it can correctly attribute text to that user.

% \noindent \textbf{Multidimensional Assessment.} Author attribution inherently involves analyzing multiple facets of text, such as vocabulary choice, sentence structure, tone, and thematic preferences. By formulating personalization as an author attribution task, we can leverage this multidimensional analysis to gauge the depth and accuracy of personalization.

% \noindent \textbf{Objective Benchmarking.} One of the challenges with personalization is its subjective nature; what feels personalized to one user might not feel the same to another. However, by relating persoanlziation evaluation to author attribution problem, we introduce an objective measure and unlock the possibility of further improving LLM as an evaluator in term of this dimension. 

\subsection{LLM as Evaluator}
For a model generated text $\hat{X}_t$ and given the immediate context $Q$ and the personal context $U_t$, {\sysname} is expected to separately evaluate the textual \textit{quality} of $\hat{X}_t$, the \textit{relevance} between $\hat{X}_t$ and $Q$, and how likely $\hat{X}_t$ is generated by the author of $U_t$. A reliable evaluator is needed to measure each of the dimensions. In the literature, without human judges, general quality of a text is often measured by statistics computed against certain reference texts or corpora (e.g., BLEU, Perplexity, and Readability), relevance is often measured by its similarity to the query, and author attribution is often predicted by a specifically trained classifier. These evaluators either fail to capture the nuances within and across these dimensions, or they require tremendous labeled data to train the classifier or as references. 

{\sysname} leverages LLMs as the evaluator.  It harnesses the expansive knowledge and reasoning capabilities of LLMs to capture the nuances in each of the facets of personalized text. Analogous to A/B testing in human evaluation, we instruct the LLM evaluator to record its preference between paired outputs rather than assigning a pointwise score to each output. We select A/B testing over individual ratings for its advantages in eliminating biases, controlling for confounders, and simplifying decision-making~\cite{carterette_preferences}. Indeed, it is much easier to decide whether A or B is more personalized than deciding to what degree A is personalized, even for human raters.

%Initially, we face the decision between pointwise and pairwise model comparison. While pointwise evaluation assesses each model in isolation, giving it a score based on certain criteria, pairwise evaluation involves directly comparing two models to determine which performs better in a given scenario.  For personalized text, the latter can be particularly effective. One of primary strengths of pairwise comparison lies in its ability to highlight the differential performance between models, eliminating any external biases that might creep in when models are evaluated individually. Additionally, by using the same evaluation set for both models, the variabilities due to external factors or inherent noise are largely neutralized, leading to a more reliable measure of their relative strengths and weaknesses. This approach is especially valuable in scenarios where models perform at similar levels; pairwise comparisons can spotlight fine-grained distinctions that might go unnoticed in isolated evaluations. Furthermore, the direct juxtaposition simplifies the decision-making process~\cite{carterette_preferences}, making it more intuitive to discern which model outperforms the other.  

Formally, given $t$, $U_t$, and $Q$, let $\hat{X}^a_t$ and $\hat{X}^b_t$ %for user $t$ with personal context $U_t$ under context $Q$ 
be two pieces of text generated by systems $a$ and $b$ respectively. We use {\sysname}$_Q$($\hat{X}^a_t$, $\hat{X}^b_t$) to denote a quality preference of the LLM evaluator between $\hat{X}^a_t$ and $\hat{X}^b_t$, which is independent of the immediate context and the personal context. Similarly, a relevance preference is denoted as {\sysname}$_R$($\hat{X}^a_t$, $\hat{X}^b_t$ | $Q$), which is conditional on $Q$, and a personalization preference is denoted as {\sysname}$_P$($\hat{X}^a_t$, $\hat{X}^b_t$ | $U_t$), which is conditional on $U_t$, the personal context or user profile of $t$. 

{\sysname}$_Q$($\hat{X}^a_t$, $\hat{X}^b_t$), {\sysname}$_R$($\hat{X}^a_t$, $\hat{X}^b_t$ | $Q$), and {\sysname}$_P$($\hat{X}^a_t$, $\hat{X}^b_t$ | $U_t$) can be obtained %Beside given samples, context and user profile, we need to craft 
through prompting the LLM to make specific comparisons between the two text samples given nothing, the immediate context $Q$, or personal examples sampled from $U_t$. Default instructions for the LLM evaluator are as follows: 
 
\begin{itemize}
    \item \textbf{Quality}: compare the provided responses and select which one is more fluent and cohesive.
    \item \textbf{Relevance}: compare the provided responses and select which one is more relevant to the given context: {$\langle Q \rangle$}.
    \item \textbf{Personalization}: compare the provided responses to select which is more likely to be written by the same author who wrote the following examples: {$\langle U_t \rangle$}. 
\end{itemize}

\noindent\textbf{Aggregating Evaluations.} To compare two generation models $a$ and $b$, we sample multiple test cases ($Q$, $t$, $U_t$) and use the LLM to evaluate the pair of their generated text examples $\hat{X}^a_t$ and $\hat{X}^b_t$ for each test case. Note that the response of an LLM may be inconsistent over repeated runs, and it is important to ensure that the order of the two example $\hat{X}^a_t$ and $\hat{X}^b_t$ does not influence the decision of the LLM evaluator. To ensure the consistency of the judgment and mitigate potential order biases, %or inconsistencies due to sample order
we repeat every evaluation for an even number of times. In half of these repeated evaluations, we present the paired examples $\hat{X}^a_t$ followed by $\hat{X}^b_t$, while in the other half, we reverse the sequence to ``$\hat{X}^b_t$ followed by $\hat{X}^a_t$.'' %By employing this strategy, we aim to guarantee that the final evaluation remains robust and is not influenced by the presentation order of the samples. This procedure is critical to ensure objective and reliable evaluations, especially when assessing subtle differences.
We then aggregate the results of all repeated evaluations to decide the ``Win,'' ``Tie'', or ``Loss'' outcome of the two competing examples ($\hat{X}^a_t$ and $\hat{X}^b_t$) for this particular test case. The outcomes over all sampled test cases are aggregated to calculate the ``Win, Tie, and Loss'' ratio for the comparison between the two systems $a$ and $b$.

\noindent\textbf{Elo Rating.} While pairwise model comparisons offer a nuanced understanding of relative model performances, they cannot paint a comprehensive picture of how multiple models rank in a broader context. To address this limitation, we leverage the Elo rating system~\cite{elo1978rating}, a method originally designed for ranking chess players, and translate the outcomes of pairwise comparisons into Elo scores. The Elo score of each contestant model represents its standing relative to its peers.  This not only offers a consolidated view to compare the performance of multiple models but also ensures that each pairwise contest contributes to an overall, unified ranking system.  In our scenario, every generation model being evaluated is a ``player'' and every sampled test case ($Q$, $t$, $U_t$) is a ``game.'' To reduce the sample order effect, we bootstrap the game orders and report the median Elo scores for a robust estimation.  More details about Elo score can be found in Appendix section.




\begin{figure*}[!ht] 
\centering
\includegraphics[width=.22\textwidth]{figs/agreement_all.png}
\includegraphics[width=.22\textwidth]{figs/agreement_truth_xl.png}
\includegraphics[width=.22\textwidth]{figs/agreement_truth_xxl.png}

\includegraphics[width=.22\textwidth]{figs/agreement_xl_xxl.png}
\includegraphics[width=.22\textwidth]{figs/agreement_xl_xxl_amazon_movie.png}
\includegraphics[width=.22\textwidth]{figs/agreement_xl_xxl_amazon_clothing.png}
\vspace{-0.3cm}
\caption{Agreement between evaluators and assumed truth (GOLD > XXL > XL) at test case level; error bars represent 95\% confidence intervals. {\sysname} is more accurate than human raters and traditional NLG metrics.} \label{figure:agreement}
\vspace{-0.3cm}
\end{figure*}



==> subfiles/results_blue_rouge.tex <==


\begin{table}[h]
\centering
\caption{Results for various models on different datasets}
\begin{tabular}{c|c|c|c|c|c}
\hline
\textbf{Dataset} & \textbf{Model Name} & \textbf{BLEU} & \textbf{ROUGE1} & \textbf{ROUGE2} & \textbf{ROUGEL} \\
\hline
\multirow{4}{*}{LaMP email} & xxl & 10.94 & 29.63 & 13.36 & 21.67 \\
                            & xl  & 10.27 & 29.70 & 13.01 & 21.42 \\
                            & large & 9.89 & 29.50 & 12.53 & 20.98 \\
                            & base & 10.33 & 27.90 & 13.08 & 21.37 \\
\hline
\multirow{4}{*}{Amazon books} & xxl & 4.82 & 29.04 & 6.84 & 17.69 \\
                              & xl  & 4.27 & 26.12 & 5.95 & 16.51 \\
                              & large & 3.67 & 23.64 & 5.06 & 15.76 \\
                              & base & 3.69 & 22.49 & 4.84 & 15.47 \\
\hline
\multirow{4}{*}{Amazon clothing} & xxl & 7.46 & 36.30 & 10.30 & 21.49 \\
                                 & xl  & 7.13 & 34.63 & 9.80 & 20.91 \\
                                 & large & 6.91 & 34.01 & 9.61 & 20.88 \\
                                 & base & 6.30 & 30.99 & 8.47 & 19.83 \\
\hline
\multirow{4}{*}{Amazon home} & xxl & 6.65 & 34.48 & 9.06 & 20.70 \\
                             & xl  & 6.35 & 32.13 & 8.51 & 19.96 \\
                             & large & 5.62 & 29.71 & 7.46 & 18.76 \\
                             & base & 5.51 & 28.18 & 7.19 & 18.72 \\
\hline
\multirow{4}{*}{Amazon movie} & xxl & 2.86 & 24.18 & 4.03 & 14.79 \\
                              & xl  & 2.47 & 20.23 & 3.26 & 13.47 \\
                              & large & 2.11 & 18.27 & 2.68 & 12.76 \\
                              & base & 1.84 & 15.94 & 2.25 & 11.97 \\
\hline
\multirow{4}{*}{Reddit} & xxl & 7.08 & 23.96 & 9.71 & 18.54 \\
                        & xl  & 7.75 & 21.58 & 9.34 & 17.86 \\
                        & large & 5.08 & 18.26 & 5.81 & 14.78 \\
                        & base & 7.50 & 19.65 & 8.72 & 17.20 \\
\hline
\end{tabular}
\end{table}



==> subfiles/results_model_comparision.tex <==

\begin{table}[h]
\centering
\caption{books}
\begin{tabular}{c|c|c|c|c|c}
\hline
Model a & Model b & Eval Dim & Win & Loss & Tie \\
\hline
\multirow{9}{*}{xxl} & xl & personalization & 62.6 & 32.4 & 5.0 \\
& xl & quality & 66.5 & 31.4 & 2.1 \\
& xl & relevance & 61.8 & 32.2 & 6.0 \\
\cline{2-6}
& large & personalization & 74.9 & 21.8 & 3.3 \\
& large & quality & 80.4 & 19.2 & 0.4 \\
& large & relevance & 70.4 & 24.5 & 5.1 \\
\cline{2-6}
& base & personalization & 77.8 & 19.4 & 2.8 \\
& base & quality & 83.7 & 15.7 & 0.6 \\
& base & relevance & 75.3 & 20.6 & 4.1 \\
\midrule
\multirow{6}{*}{xl} & large & personalization & 62.6 & 32.6 & 4.8 \\
& large & quality & 68.2 & 29.7 & 2.1 \\
& large & relevance & 59.5 & 34.1 & 6.4 \\
\cline{2-6}
& base & personalization & 68.3 & 27.5 & 4.2 \\
& base & quality & 73.4 & 25.6 & 1.0 \\
& base & relevance & 63.5 & 31.7 & 4.8 \\
\midrule
\multirow{3}{*}{large} & base & personalization & 55.7 & 38.3 & 6.0 \\
& base & quality & 56.8 & 40.9 & 2.3 \\
& base & relevance & 52.9 & 41.0 & 6.1 \\
\hline
\end{tabular}
\end{table}


\begin{table}[!h]
\centering
\caption{clothing}
\begin{tabular}{c|c|c|c|c|c}
\hline
Model a & Model b & Eval Dim & Win & Loss & Tie \\
\hline
\multirow{9}{*}{xxl} & xl & personalization & 59.9 & 33.8 & 6.3 \\
& xl & quality & 68.5 & 29.3 & 2.2 \\
& xl & relevance & 56.6 & 38.4 & 5.0 \\
\cline{2-6}
& large & personalization & 66.8 & 28.3 & 4.9 \\
& large & quality & 75.9 & 22.4 & 1.7 \\
& large & relevance & 59.6 & 35.1 & 5.3 \\
\cline{2-6}
& base & personalization & 74.4 & 20.4 & 5.2 \\
& base & quality & 88.8 & 9.8 & 1.4 \\
& base & relevance & 71.5 & 25.0 & 3.5 \\
\midrule
\multirow{6}{*}{xl} & large & personalization & 53.4 & 38.7 & 7.9 \\
& large & quality & 58.9 & 38.7 & 2.4 \\
& large & relevance & 50.6 & 43.1 & 6.3 \\
\cline{2-6}
& base & personalization & 67.8 & 27.3 & 4.9 \\
& base & quality & 79.3 & 19.2 & 1.5 \\
& base & relevance & 66.1 & 30.5 & 3.4 \\
\midrule
\multirow{3}{*}{large} & base & personalization & 62.4 & 32.1 & 5.5 \\
& base & quality & 75.0 & 23.6 & 1.4 \\
& base & relevance & 61.4 & 32.9 & 5.7 \\
\hline
\end{tabular}
\end{table}

\begin{table}[!h]
\centering
\caption{home}
\begin{tabular}{c|c|c|c|c|c}
\hline
Model a & Model b & Eval Dim & Win & Loss & Tie \\
\hline
\multirow{9}{*}{xxl} & xl & personalization & 63.4 & 29.1 & 7.5 \\
& xl & quality & 67.7 & 29.5 & 2.8 \\
& xl & relevance & 58.7 & 35.1 & 6.2 \\
\cline{2-6}
& large & personalization & 74.9 & 19.9 & 5.2 \\
& large & quality & 81.4 & 17.4 & 1.2 \\
& large & relevance & 69.4 & 26.3 & 4.3 \\
\cline{2-6}
& base & personalization & 82.3 & 14.2 & 3.5 \\
& base & quality & 88.1 & 11.0 & 0.9 \\
& base & relevance & 77.8 & 18.3 & 3.9 \\
\midrule
\multirow{6}{*}{xl} & large & personalization & 60.7 & 35.2 & 4.1 \\
& large & quality & 65.1 & 32.7 & 2.2 \\
& large & relevance & 58.1 & 36.3 & 5.6 \\
\cline{2-6}
& base & personalization & 69.6 & 26.1 & 4.3 \\
& base & quality & 76.6 & 22.4 & 1.0 \\
& base & relevance & 65.6 & 30.1 & 4.3 \\
\midrule
\multirow{3}{*}{large} & base & personalization & 59.5 & 35.3 & 5.2 \\
& base & quality & 62.3 & 35.4 & 2.3 \\
& base & relevance & 58.4 & 35.6 & 6.0 \\
\hline
\end{tabular}
\end{table}

\begin{table}[!htb]
\centering
\caption{movie}
\begin{tabular}{c|c|c|c|c|c}
\hline
Model a & Model b & Eval Dim & Win & Loss & Tie \\
\hline
\multirow{9}{*}{xxl} & xl & personalization & 68.0 & 27.8 & 4.2 \\
& xl & quality & 71.9 & 26.8 & 1.3 \\
& xl & relevance & 69.0 & 26.5 & 4.5 \\
\cline{2-6}
& large & personalization & 76.4 & 20.3 & 3.3 \\
& large & quality & 82.4 & 16.5 & 1.1 \\
& large & relevance & 76.6 & 19.0 & 4.4 \\
\cline{2-6}
& base & personalization & 82.2 & 15.4 & 2.4 \\
& base & quality & 89.5 & 9.8 & 0.7 \\
& base & relevance & 81.9 & 14.5 & 3.6 \\
\midrule
\multirow{6}{*}{xl} & large & personalization & 59.8 & 34.9 & 5.3 \\
& large & quality & 62.8 & 34.6 & 2.6 \\
& large & relevance & 59.3 & 35.3 & 5.4 \\
\cline{2-6}
& base & personalization & 71.2 & 25.6 & 3.2 \\
& base & quality & 76.0 & 21.8 & 2.2 \\
& base & relevance & 67.5 & 25.0 & 7.5 \\
\midrule
\multirow{3}{*}{large} & base & personalization & 58.4 & 35.4 & 6.2 \\
& base & quality & 62.8 & 34.2 & 3.0 \\
& base & relevance & 57.7 & 35.1 & 7.2 \\


\hline
\end{tabular}
\end{table}

\begin{table}[!h]
\centering
\caption{reddit}
\begin{tabular}{c|c|c|c|c|c}
\hline
Model a & Model b & Eval Dim & Win & Loss & Tie \\
\hline
\multirow{9}{*}{xxl} & xl & personalization & 67.1 & 28.6 & 4.3 \\
& xl & quality & 71.7 & 26.9 & 1.4 \\
& xl & relevance & 65.4 & 29.2 & 5.4 \\
\cline{2-6}
& large & personalization & 80.4 & 17.9 & 1.7 \\
& large & quality & 80.4 & 18.2 & 1.4 \\
& large & relevance & 71.0 & 24.2 & 4.8 \\
\cline{2-6}
& base & personalization & 84.6 & 13.7 & 1.7 \\
& base & quality & 83.3 & 15.7 & 1.0 \\
& base & relevance & 74.4 & 21.6 & 4.0 \\
\midrule
\multirow{6}{*}{xl} & large & personalization & 60.2 & 36.1 & 3.7 \\
& large & quality & 59.7 & 37.7 & 2.6 \\
& large & relevance & 51.2 & 41.1 & 7.7 \\
\cline{2-6}
& base & personalization & 72.2 & 24.9 & 2.9 \\
& base & quality & 66.6 & 31.1 & 2.3 \\
& base & relevance & 59.9 & 33.8 & 6.3 \\

\midrule
\multirow{3}{*}{large} & base & personalization & 59.7 & 36.7 & 3.6 \\
& base & quality & 59.3 & 39.3 & 1.4 \\
& base & relevance & 53.2 & 38.6 & 8.2 \\
\hline
\end{tabular}
\end{table}
\begin{table}[ht]
\centering
\caption{LaMP}
\begin{tabular}{c|c|c|c|c|c}
\hline
Model a & Model b & Eval Dim & Win & Loss & Tie \\
\hline
\multirow{9}{*}{xxl} & xl & personalization & 52.13 & 41.71 & 6.16 \\
& xl & quality & 61.14 & 36.97 & 1.90 \\
& xl & relevance & 54.50 & 42.65 & 2.84 \\
\cline{2-6}
& large & personalization & 55.45 & 41.23 & 3.32 \\
& large & quality & 64.93 & 34.12 & 0.95 \\
& large & relevance & 55.92 & 42.65 & 1.42 \\
\cline{2-6}
& base & personalization & 64.93 & 32.70 & 2.37 \\
& base & quality & 73.93 & 24.64 & 1.42 \\
& base & relevance & 63.51 & 33.65 & 2.84 \\
\midrule
\multirow{6}{*}{xl} & large & personalization & 45.97 & 47.39 & 6.64 \\
& large & quality & 55.45 & 41.23 & 3.32 \\
& large & relevance & 48.82 & 47.87 & 3.32 \\
\cline{2-6}
& base & personalization & 59.24 & 36.02 & 4.74 \\
& base & quality & 63.51 & 33.18 & 3.32 \\
& base & relevance & 59.24 & 39.34 & 1.42 \\
\midrule
\multirow{3}{*}{large} & base & personalization & 55.92 & 36.02 & 8.06 \\
& base & quality & 56.40 & 41.23 & 2.37 \\
& base & relevance & 57.35 & 40.28 & 2.37 \\


\hline
\end{tabular}
\end{table}

